Pydrofoil: accelerating Sail-based instruction set simulators

We present Pydrofoil, a multi-stage compiler that generates instruction set simulators (ISSs) from processor instruction set architectures (ISAs) expressed in the high-level, verification-oriented ISA specification language Sail. Pydrofoil shows a > 230x speedup over the C-based ISS generated by Sail on our benchmarks, and is based on the following insights. (i) An ISS is effectively an interpreter loop, and tracing just-in-time (JIT) compilers have proven effective at accelerating those, albeit mostly for dynamically typed languages. (ii) ISS workloads are highly atypical, dominated by intensive bit manipulation operations. Conventional compiler optimisations for general-purpose programming languages have limited impact for speeding up such workloads. We develop suitable domain-specific optimisations. (iii) Neither tracing JIT compilers, nor ahead-of-time (AOT) compilation alone, even with domain-specific optimisations, suffice for the generation of performant ISSs. Pydrofoil therefore implements a hybrid approach, pairing an AOT compiler with a tracing JIT built on the meta-tracing PyPy framework. AOT and JIT use domain-specific optimisations. Our benchmarks demonstrate that combining AOT and JIT compilers provides significantly greater performance gains than using either compiler alone.

==> measurements/arm.tex <==
\begin{tabular}{lrrr}
\toprule
Implementation & time & KIPS & speedup \\
\midrule
pydrofoil-arm & 15.2 & 1618.2 & 69.4 \\
pydrofoil-arm-no-jit & 54.3 & 452.9 & 19.4 \\
sail-arm & 1055.9 & 23.3 & 1.0 \\
\bottomrule
\end{tabular}


==> measurements/cheriot.tex <==
\begin{tabular}{lrrr}
\toprule
Implementation & time & KIPS & speedup \\
\midrule
pydrofoil-cheriot & 13.8 & 19912.6 & 51.9 \\
pydrofoil-cheriot-no-jit & 31.1 & 8840.8 & 23.0 \\
sail-cheriot & 715.2 & 384.0 & 1.0 \\
\bottomrule
\end{tabular}


==> measurements/sail-comparison.tex <==
{\small
\begin{tabular}{lrrrr}
\toprule
 & \multicolumn{2}{c}{KIPS} & \multicolumn{2}{c}{slowdown} \\
Benchmark & mcf.0 & perlbench.0 & mcf.0 & perlbench.0 \\
Implementation &  &  &  &  \\
\midrule
full & 22320.79 & 15203.28 & 1.00 & 1.00 \\
no-jit & 1820.04 & 1776.76 & 12.26 & 8.56 \\
sail-risc-v* & 95.63 & 59.60 & 233.40 & 255.08 \\
\bottomrule
\end{tabular}
}

